Fast Neural Network Verification via Shadow Prices

To use neural networks in safety-critical settings it is paramount to provide assurances on their runtime operation. Recent work on ReLU networks has sought to verify whether inputs belonging to a bounded box can ever yield some undesirable output. Input-splitting procedures, a particular type of verification mechanism, do so by recursively partitioning the input set into smaller sets. The efficiency of these methods is largely determined by the number of splits the box must undergo before the property can be verified. In this work, we propose a new technique based on shadow prices that fully exploits the information of the problem yielding a more efficient generation of splits than the state-of-the-art. Results on the Airborne Collision Avoidance System (ACAS) benchmark verification tasks show a considerable reduction in the partitions generated which substantially reduces computation times. These results open the door to improved verification methods for a wide variety of machine learning applications including vision and control.

==> sections/polytopicpartitons.tex <==
\section{Polytopic Partitions Induced by ReLU Networks}
\label{sec:polytopic_partitions_induced_byReLU}

In this section we will introduce some geometrical properties of ReLU networks that will be important for the remainder of the paper. We begin by showing how the domain of a ReLU network is divided into polytopic regions which are induced by the weight matrices and bias vectors. 

\subsection{Affine Transformations and Polytopic Partitions}
\label{subsec:affine_transform_polytopic_p}

For $x_1 \in \mathbb{R}^{n_1}$ and $W \in \mathbb{R}^{n_2 \times n_1}$ and the affine transformation $\hat x_2 = Wx_1 + b$, one can view the rows of matrix $W$ as the normal vectors of a set of hyperplanes with bias $b$, and $\hat x_2$ as a distance of $x_1$ to each hyperplane (scaled by some constant). Furthermore, the sign of the entries of $y$ shows whether a point is in the negative or positive half of the associated half-space. Hence, the tuple $(W,b)$ induces a (signed) partition of the domain into polytopic regions, where the interior of each polytopic region contains points whose affine transformations have the same sign element-wise. Figure \ref{regions_affine} shows a typical partition in $\mathbb{R}^2$.

\begin{figure}[ht]
\begin{center}
\centerline{\includegraphics[scale = 0.3]{icml2018/figures/regions.png}} %width=\columnwidth,
\caption{A typical partition induced by an affine transformation with $W \in \mathbb{R}^{3\times 2}$ and $b \in \mathbb{R}^{3}$. The hyperplanes are assumed to be in general position.}
\label{regions_affine}
\end{center}
\end{figure}

\subsection{Image under the Rectifier Function}
\label{subsec:rectifier_partitions}

It is interesting to see how the composition of a non-linear function and an affine transformation affect the output as $x_1$ varies. In particular, the rectifier function is defined as ${r(x) := \max\{0,x\}}$ element-wise, and the composition is ${x_2 = r(Wx_1+b)}$. With the partition of the domain form Fig. \ref{regions_affine} in mind, in the space of $x_2$, region \textbf{A} gets mapped to a point in the origin, whereas region \textbf{B} gets mapped to a line segment and regions \textbf{C} and \textbf{D} get mapped to unbounded 2D polytopes. Figure \ref{regions_transformed} illustrates the resulting transformation from $x_1$ to $x_2$. More generally, each of the polytopic regions induced by $(W,b)$ is mapped to a polytope in the space of $x_2$ of dimension at most $\underbar{$n$} = \min\{n1,n2\}$. 

\begin{figure}[ht]
\begin{center}
\centerline{\includegraphics[scale = 0.2]{icml2018/figures/transform.png}} %width=\columnwidth,
\caption{Visualization of the image of $x_1$ after the affine and non-linear ReLU tranformation. From the seven regions in the space of $x_1$, one gets mapped to a point (the origin), three get mapped to line segments and three get mapped to 2D polytopes in $\mathbb{R}^3$.}
\label{regions_transformed}
\end{center}
\end{figure}

\subsection{ReLU Network: A Piece-wise Affine Function}
\label{subsec:relu_definition}

Let $f_\theta(x)$ be a ReLU network defined by
\begin{equation}
\label{eq:relu}
\begin{split}
  & \hat{z}_{i+1} = W_i z_i + b_i, ~ \text{for} ~ i=1,...,K-1 \\
  & z_j = \max\{\hat{z}_j,0\},  ~ \text{for} ~ j=2,...,K-1 \\
\end{split}
\end{equation}
with $W_i \in \mathbb{R}^{n_{i+1} \times n_i}$, $b \in \mathbb{R}^{n_{i+1}}$, $z_1 = x \in \mathcal{B}$, where $\mathcal{B}$ is a bounded box in $\mathbb{R}^{n_1}$ and $f_\theta(x) = \hat{z}_{K}$. The set $\theta = \{W_i,b_i\}_{i=1,...,K-1}$ represents the set of weights of the network.

This network is but a composition of the transformations presented in Sec. \ref{subsec:affine_transform_polytopic_p} and \ref{subsec:rectifier_partitions}. Geometrically, this implies that as $K$ grows larger more partitions will be generated in the input space. Figure 2(b)

Finally, it is important to mention that $\bar y$ is a piecewise affine function. One can immediately see that by noting that the composition of a piecewise linear function (the rectifier) and an affine function, results in a piecewise affine function. Alternatively, one can see this by rewriting the equation for $\bar y$ as a matrix vector product as done in [ref]:

\begin{equation}
\bar y = r(Wx + b) = D(Wx+b)
\end{equation}

with $D = diag(\textbf{1}\{Wx+b \geq 0\})$ and $\textbf{1}\{z \geq 0\}$ is the element-wise indicator function. Thus, for $x$ belonging to some polytopic region induced by $(W,b)$, $D$ is a constant and $\bar y = DWx + Db$ is affine (i.e. $\frac{\partial \bar y}{\partial x}$ will be constant).

\subsection{Exact Image Computation}

As seen thus far, ReLU networks are piece-wise affine functions. A possible way of verifying some property of the image would be to find all the polytopic regions within the input hyper-box, and then mapping them through their corresponding affine transformation. Each transformed region can then be checked individually. Unfortunately, as shown in \cite{Pascanu13,montufar2014number,Serra17}, the number of regions can grow exponentially fast with the input dimension and the depth of the network, and approaches such as this one become impractical.
